A journey in modal proof theory: From minimal normal modal logic to discrete linear temporal logic

Extending and generalizing the approach of 2-sequents (Masini, 1992), we present sequent calculi for the classical modal logics in the K, D, T, S4 spectrum. The systems are presented in a uniform way-different logics are obtained by tuning a single parameter, namely a constraint on the applicability of a rule. Cut-elimination is proved only once, since the proof goes through independently from the constraints giving rise to the different systems. A sequent calculus for the discrete linear temporal logic ltl is also given and proved complete. Leitmotiv of the paper is the formal analogy between modality and first-order quantification.

==> constructivism.tex <==
\section{Constructivism and modal types}\label{sec:constructivism}
{\rosso{
\textbf{la base e' quella del papero martini-masini \cite{MM:ComInt:95}. Dovrebbe essere semplice dare lambda calcolo tipato, seguendo le linee del lambda calcolo alla Church per il sistema P del cubo di Barendregt.
}
}


==> global.tex <==
% -*- Mode: LaTeX -*- 
% Time-stamp:  <global.tex 02/11/20 10:57:17 guerrini@sgport.dsi.uniroma1.it> 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  Packages

%\usepackage{latexsym}
\usepackage{amsmath,amssymb}
\usepackage{eucal}
\usepackage{euler}
\usepackage{xspace}
\usepackage{stmaryrd}

%%  xy-pic
\usepackage{xy}
\xyoption{frame}
\xyoption{arrow}
\xyoption{curve}
\xyoption{arc}
\xyoption{line}
\xyoption{matrix}
\xyoption{tile}
\xyoption{ps}
\xyoption{dvips}
\xyoption{color}
  % xy-macros
%  \input{xy-nets}
%  \boldnodestrue
%  \newlength\vsgraphunit \vsgraphunit=4ex
%  \newlength\hsgraphunit \hsgraphunit=8ex
%  %%%  XY-pic/qsymbols patch from Kris Rose
%  {\makeatletter \gdef\noqmagic{\def\inxy@{TF}}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  Theorem-like environments

\usepackage{amsthm}

\theoremstyle{plain}
    \newtheorem{theorem}{Theorem}
    \newtheorem{lemma}[theorem]{Lemma}
    \newtheorem{corollary}[theorem]{Corollary}
    \newtheorem{proposition}[theorem]{Proposition}
%    \newtheorem{criterion}{Criterion}[section]
%    \newtheorem{algorithm}{Algorithm}[section]
    \newtheorem{fact}[theorem]{Fact}
\theoremstyle{definition}
    \newtheorem{definition}[theorem]{Definition}
%    \newtheorem{conjecture}{Conjecture}[section]
%    \newtheorem{example}{Example}[section]
%    \newtheorem{problem}{Problem}[section]
\theoremstyle{remark}
    \newtheorem{remark}[theorem]{Remark}
%        \renewcommand{\theremark}{}
%    \newtheorem{notation}{Notation}[section]
%%        \renewcommand{\thenotation}{}
%%    \newtheorem{note}{Note}[section]
%%        \renewcommand{\thenote}{}
%%    \newtheorem{claim}{Claim}[section]
%    \newtheorem{summary}{Summary}
%        \renewcommand{\thesummary}{}
%    \newtheorem{synopsis}{Synopsis}
%        \renewcommand{\thesynopsis}{}
%%    \newtheorem{case}{Case}[section]
%%    \newtheorem{ack}{Acknowledgement}[section]
%%        \renewcommand{\theack}{}
\theoremstyle{plain}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  Prooftree

% in latex2e occorre definire "il contatore mscount"
\newcount\mscount
\input{prooftree}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  Macros

\newcommand{\ie}{\emph{i.e.}\xspace}
\newcommand{\eg}{\emph{e.g.}\xspace}

% Rules

\newcommand{\linea}{\leavevmode\hrule\mbox{}}
\newcommand{\dlinea}{\leavevmode\hrule\vspace{1pt}\hrule\mbox{}}

==> local.tex <==
% -*- Mode: LaTeX -*- 
% Time-stamp:  <local.tex 03/03/20 13:26:52 guerrini@zambujero.lan.home> 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  Packages

% ...


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  Formato pagina

% Dimensioni orizzontali
% --- 1st set ---
%\oddsidemargin  -0.185in     %   Left margin on odd-numbered pages.
%\evensidemargin -0.185in     %   Left margin on even-numbered pages.
%\textwidth 6.675in          %   Width of text line.
%\marginparwidth .75in       %   Width of marginal notes.
% --- 2nd set ---
%\oddsidemargin  -0.4in     %   Left margin on odd-numbered pages.
%\evensidemargin -0.4in     %   Left margin on even-numbered pages.
%\textwidth 7in          %   Width of text line.

% Dimensioni verticali
% --- 1st det ---
%\topmargin -.35in
%\textheight 9.5in
%% --- 2nd set ---
%\topmargin -.5in
%%\textheight 9.8in

%%%% I prefer paragraphs spaced rather than indented
%\parindent=0pt
%\parskip=4pt plus 2pt minus 1pt


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  Macro

%%%%\mathcode`\;="263B  % make ; a binary operator & bold (for composition)
\mathcode`\<="4268  % < = \langle
\mathcode`\>="5269  % > = \rangle
% \mathcode`\.="313A  % make . a binary  relation

%\mathchardef\semicolon="603B % the original
\mathchardef\gt="313E
\mathchardef\lt="313C


%%%%%%%%%%%%%%%%%%%%
% Sequenti

\newcommand{\seqsym}{\vdash}
\newcommand{\varseqsym}{%
  \mathrel{%
    \vrule height 1ex width 0.3ex depth -.1ex
    \mkern-3mu
    \smash-}}

\newcommand{\seq}[2]{#1 \seqsym #2} % sequente a due lati
\newcommand{\rseq}[1]{\seqsym #1} % sequente solo destra
\newcommand{\lseq}[1]{#1 \seqsym} % sequente solo destra

%\newcommand{\vseq}[1]{\begin{array}{c} #1\end{array}} % due sequenza

%%%%%%%%%%%%%%%%%%%%
% Regole dimostrazioni

\newcommand{\Urule}[3]{%
  \prooftree #1 \Justifies #2 \using #3 \endprooftree}
\newcommand{\urule}[3]{%
  \prooftree #1 \justifies #2 \using #3 \endprooftree}
\newcommand{\brule}[4]{%
  \prooftree #1\ \ \ #2 \justifies #3 \using #4 \endprooftree}
\newcommand{\trule}[5]{%
  \prooftree #1\ \ \ #2 \ \ #3\justifies #4 \using #5 \endprooftree}
\newcommand{\lto}[2]{%
  \prooftree #2 \leadsto #1 \endprooftree}
\newcommand{\LT}[3]{%
  \prooftree #2 \leadsto #1 \using #3\endprooftree}
\newcommand{\stackpr}[2]{\stackrel{\mbox{$#1$}}{#2}}

%%%%%%%%%%%%%%%%%%%%
% Connettivi e nomi regole

%\def\lbx{\,!}

\newcommand{\ax}{\mathsf{ax}}
\newcommand{\cut}{\mathsf{cut}}
\newcommand{\foc}{\mathsf{foc}}
\newcommand{\defoc}{\mathsf{defoc}}
\newcommand{\der}{\mathsf{der}}
\newcommand{\prom}{\mathsf{prom}}
\newcommand{\weak}{\mathsf{weak}}
\newcommand{\contr}{\mathsf{contr}}
%\newcommand{\mux}{\mathsf{mux}}
%\newcommand{\demux}{\mathsf{demux}}
\newcommand{\lpar}{\mathbin{\bindnasrepma}} % linear par
\newcommand{\tens}{\varotimes} % tensor
\newcommand{\limp}{\multimap} % linear implication
\newcommand{\llimp}{\limp} % sinonimo per linear implication
\newcommand{\liff}{\circ--\circ} % linear iff
\newcommand{\plus}{\varoplus} % plus
\newcommand{\with}{\mathbin{\binampersand}} % linear with

\newcommand{\imp}{\to} % implication
\newcommand{\varimp}{\supset} % third implication
\newcommand{\aimp}{% anti implication
%  \overline{\makebox[0pt]{$\;\,\imp$}\ }}
  \bar{\imp}}
\newcommand{\ut}{\lor} % or
\newcommand{\aut}{\bar{\ut}} % anti or
\newcommand{\et}{\land} % and
\newcommand{\aet}{\bar{\et}} % anti and
\newcommand{\aneg}{% anti neg
%  \overline{\makebox[0pt]{$\;\,\lnot$}\ }}
  \bar{\lnot}}
\newcommand{\abot}{\bar{\perp}} % anti bottom
\newcommand{\focsym}{\downarrow}
\newcommand{\defocsym}{\uparrow}
\newcommand{\mneg}{\sim\!\!}

\newcommand{\impI}{\imp\mathcal{I}}
\newcommand{\orI}{\ut\mathcal{I}}
\newcommand{\iorI}[1]{\ut\mathcal{I}_{#1}}
\newcommand{\andI}{\et\mathcal{I}}
\newcommand{\iandI}[1]{\et\mathcal{I}_{#1}}
\newcommand{\negI}{\lnot\mathcal{I}}
\newcommand{\impE}{\imp\mathcal{E}}
\newcommand{\orE}{\ut\mathcal{E}}
\newcommand{\iorE}[1]{\ut\mathcal{E}_{#1}}
\newcommand{\andE}{\et\mathcal{E}}
\newcommand{\iandE}[1]{\et\mathcal{E}_{#1}}
\newcommand{\negE}{\lnot\mathcal{E}}

%%%%%%%%%%%%%%%%%%%%
% Indici ed altre marcature formule

%\newcommand{\lus}[4]{#1[ #2\vdash #3 ] #4}
\newcommand{\anti}[1]{\overline{#1}}
\newcommand{\iif}[2]{#1^{#2}}
\newcommand{\iaf}[2]{\iif{{\anti{#1}}}{#2}}
\newcommand{\rf}[1]{#1{}\,^{\makebox[0pt]{$\scriptscriptstyle{r}$}}}
\newcommand{\lf}[1]{#1{}\,^{\makebox[0pt]{$\scriptscriptstyle{l}$}}}

\newcommand{\pf}[1]{#1^\bullet}

%%%%%%%%%%%%%%%%%%%%
% Costanti della deduzione naturale

%\newcommand{\ftop}{\Ydown}
%\newcommand{\fbot}{\Yup}
\newcommand{\ftop}{\curlyvee}
\newcommand{\fbot}{\curlywedge}

\newcommand{\ydash}{\Yleft}
%\newcommand{\dderiv}{\prec}

\newcommand{\dimp}{\leftarrowtail}

%%%%%%%%%%%%%%%%%%%%
% Costanti del calcolo di termini

\newcommand{\inj}{\mathsf{in}}
\newcommand{\match}{\mathsf{match}}
\newcommand{\mwith}{\mathsf{with}}
\newcommand{\msep}{\mathsf{or}}
\newcommand{\close}{\mathsf{close}}
\newcommand{\eval}{\mathsf{eval}}
\newcommand{\apply}{\mathsf{apply}}
\newcommand{\matchwith}[4]{%
  \match\,#2\,\mwith\,\inj_1 #1_1 \mapsto #3\,\msep\,\inj_2 #1_2 \mapsto #4}
\newcommand{\closure}[2]{\close\,#1.#2}
\newcommand{\evaluate}[1]{\eval\,#1}
\newcommand{\comb}[2]{\apply\,#1\,#2}
\newcommand{\letin}[3]{%
  \mathsf{let}\ #1\ \mathsf{be}\ #2\ \mathsf{in}\ #3}


%%%%%%%%%%%%%%%%%%%%
% Traduzioni

\newcommand{\trdueseq}[1]{\left[ #1 \right]^{\sharp}}
\newcommand{\trdueseqnew}[1]{\left[ #1 \right]^{\flat}}
\newcommand{\trmin}[1]{\left[ #1 \right]^{\ast}}

%%%%%%%%%%%%%%%%%%%%
% Acronimi e altri nomi

%\newcommand{\LL}{\mathsf{LL}}
%\newcommand{\TWOLL}{\mathsf{2LL}}
%\newcommand{\LLL}{\mathsf{LLL}}
%\newcommand{\TWOLLL}{\mathsf{2LLL}}
%\newcommand{\ELL}{\mathsf{ELL}}
%\newcommand{\TWOELL}{\mathsf{2ELL}}
%\newcommand{\SFOUR}{\mathsf{S4}}
%\newcommand{\KD}{\mathsf{KD}}
\newcommand{\MELL}{\textsf{MELL}\xspace}
%\newcommand{\SLL}{\mathsf{LL+S}}
%\newcommand{\TWOSLL}{\mathsf{2SLL}}
\newcommand{\FLC}{\textsf{FoLK}\xspace}
\newcommand{\FNC}{\textsf{FoNK}\xspace}
\newcommand{\MND}{\textsf{mND}\xspace}

%%%%%%%%%%%%%%%%%%%%
% Relazioni e funzioni

\newcommand{\entails}[1]{\vdash_{\!\!\scriptscriptstyle#1}}
\newcommand{\maxlev}[1]{\max(#1)}
\newcommand{\FV}[1]{\mathsf{FV}(#1)}
\newcommand{\FA}[1]{\mathsf{FA}(#1)}
\newcommand{\FN}[1]{\mathsf{FN}(#1)}
\newcommand{\spine}[1]{\mathsf{sp}(#1)}
\newcommand{\pn}[1]{\mathcal{#1}}
\newcommand{\trll}[1]{[ #1 ]}
\newcommand{\trfc}[1]{( #1)^\sharp }
\newcommand{\trcf}[1]{( #1)^\circ }
\newcommand{\ptrll}[1]{|#1|}
\newcommand{\deriv}[1]{\mathcal{#1}}
\newcommand{\edge}{%
  \mathrel{\vbox{\hbox{${\frown}$}\vspace{-2ex}\hbox{}\vspace{-.5ex}}}}
%\newcommand{\dotedge}{%
%  \mathrel{\vbox{\hbox{${\frown}$}\vspace{-2ex}\hbox{\hspace{.9ex}$\smash\cdot$}\vspace{-.5ex}}}}
\newcommand{\noedge}{%
  \mathrel{\vbox{\hbox{${\smile}$}\vspace{-2ex}\hbox{}\vspace{-.5ex}}}}

%%% maps from proof to graphs and vice versa
%\newcommand{\graphof}[1]{\mathfrak{G}(#1)}
\newcommand{\netof}[1]{\mathfrak{N}(#1)}

%%%%%%%%%%%%%%%%%%%%
% Relazioni riduzione

\newcommand{\redto}{\to}
\newcommand{\ctr}{\triangleright}
\newcommand{\rredto}{\stackrel{*}{\redto}}
\newcommand{\cutred}{\to}
\newcommand{\mredto}{\to_m}
\newcommand{\mctr}{\triangleright_m}
\newcommand{\mrredto}{\stackrel{*}{\redto_mm}}


%%% Links: in text

\newcommand{\link}{\vartriangleright}
%\newcommand{\rootlink}{\stackrel{_0}{\link}}
%\newcommand{\unlink}{\stackrel{_1}{\link}}
%\newcommand{\binlink}{\stackrel{_2}{\link}}
%\newcommand{\unbinlink}{\stackrel{_{1,2}}{\link}}
%\newcommand{\starlink}{\stackrel{_*}{\link}}

\newcommand{\namedlink}[1]{\stackrel{\scriptscriptstyle{#1}}{\link}}

\newcommand{\axlink}{\namedlink{\ax}}
\newcommand{\cutlink}{\namedlink{\cut}}
\newcommand{\implink}{\namedlink{\imp}}
\newcommand{\utlink}{\namedlink{\ut}}
\newcommand{\etlink}{\namedlink{\et}}
\newcommand{\neglink}{\namedlink{\lnot}}
\newcommand{\boxlink}{\namedlink{\square}}

\newcommand{\weaklink}{\namedlink{\textsf{w}}}
\newcommand{\contrlink}{\namedlink{\textsf{c}}}
\newcommand{\abotlink}{\namedlink{\abot}}

%%% Links: in xy-pic

\newdimen\netunit
  \netunit=1em
\newlength\vt\newlength\hz
  \vt=1.5\netunit
  \hz=3\netunit

\newcommand{\prf}{\POS *\frm<\jot>{-}}

%\def\linkdot{\object{\POS*\frm<2pt>{*}}\POS}
%\def\linkline{\connect\dir{-} \POS ?</8pt/}
%\def\unarc{%
%  \POS @+, s2; s1, {\ellipse![[s0;s2]]_,_,![[s0;s1]]_{-}}, @-\POS}
%\def\binarc{%
%  \POS @+, s2; s1, {\ellipse![[s0;s2]]_,_,![[s0;s1]]_{=}}, @-\POS}
%\def\toplink#1{\Toplink{#1}{1}}
%\def\hsmtoplink#1{\Toplink{#1}{.5}}
%\def\hToplink#1#2{%
%  \save\POS
%  *!Ch\xybox{%
%    /l#2\netunit/ \ar@*{[|<3pt>][roundcap]}@{-} /r#2\netunit/
%    }="TOP#1",
%  "TOP#1"!L+/r\jot/="TOP#1-L",
%  "TOP#1"!R+/l\jot/="TOP#1-R" 
%  \restore\POS
%  }
%\def\Toplink#1#2{%
%  \save\POS
%  *!C\xybox{%
%    /l#2\netunit/ \ar@*{[|<3pt>][roundcap]}@{-} /r#2\netunit/
%    }="TOP#1",
%  "TOP#1"!L+/r\jot/="TOP#1-L",
%  "TOP#1"!R+/l\jot/="TOP#1-R" 
%  \restore\POS
%  }
%\def\bottomlink#1{%
%  \save\POS*!C\xybox{%
%    /l.25\netunit/ \ar@*{[|<3pt>][roundcap]}@{-} /r.25\netunit/
%    }="BOTTOM#1"\restore\POS
%  }

%\def\gbottomlink#1{%
%  \save\POS*!C\xybox{%
%%    /l.25\netunit/ \ar@*{[|<3pt>][gray][roundcap]}@{-} /r.25\netunit/
%    *=<.5\netunit,3pt>{},*\frm<2pt>{-}
%    }="BOTTOM#1"\restore\POS
%  }

%\newcommand{\net}[2]{%
%  \save\POS
%  *!C\xybox{%
%    0 \ar@*{[|<3pt>][roundcap]}@{-} /r#2\netunit/
%    }="NET#1",
%  "NET#1"!L+/r\jot/="NET#1-L",
%  "NET#1"!R+/l\jot/="NET#1-R" 
%  \restore\POS
%  }

%\newcommand{\nnet}[3]{%
%  \save\POS\net{#1}{#2}
%  "NET#1-L"+/u\jot/*!D{_#3}
%  \restore\POS
%  }

%\newcommand{\bnet}[2]{%
%  \save\POS\net{#1}{#2}
%  "NET#1-L"+/u\jot/*!D{_\textsf{box}}
%  \restore\POS
%  }

\newcommand{\lbox}[3]{%
  \save\POS 
  c.{c+<-#2\hz,#3\vt>}!C*[thicker]\frm{-}="BOX#1",
  +UL*+!DL{\scriptscriptstyle\mathsf{box}},
  \restore\POS
  }

\newcommand{\LBOX}[5]{%
  \save\POS
  *+{#4}="BOX#1-1" \prf,
  "BOX#1-1"+UR \lbox{#1}{#2}{#3},
  "BOX#1"+DL.{"BOX#1-1"+0}!DL+R(.3)*+{#5}="BOX#1-2"
  \restore\POS
  }

\newcommand{\rbox}[3]{%
  \save\POS 
  c.{c+<#2\hz,#3\vt>}!C*[thicker]\frm{-}="BOX#1",
  +UL*+!DL{\scriptscriptstyle\mathsf{box}},
  \restore\POS
  }

\newcommand{\RBOX}[5]{%
  \save\POS
  *+{#4}="BOX#1-1" \prf,
  "BOX#1-1"+UL \rbox{#1}{#2}{#3},
  "BOX#1"+DR.{"BOX#1-1"+0}!DR+L(.3)*+{#5}="BOX#1-2"
  \restore\POS
  }

\newcommand{\lpnet}[3]{%
  \save\POS
  c.{c+<-#2\hz,#3\vt>}!C*\frm<\jot>{-}="NET#1",
  \restore\POS
  }

\newcommand{\rpnet}[3]{%
  \save\POS
  c.{c+<#2\hz,#3\vt>}!C*\frm<\jot>{-}="NET#1",
  \restore\POS
  }

\newcommand{\LPNET}[5]{%
  \save\POS
  *+{#4}="NET#1-1",
  "NET#1-1"+UR \lpnet{#1}{#2}{#3},
  "NET#1"+DL.{"NET#1-1"+0}!DL+R(.3)*+{#5}="NET#1-2"
  \restore\POS
  }

\newcommand{\RPNET}[5]{%
  \save\POS
  *+{#4}="NET#1-1",
  "NET#1-1"+UL \rpnet{#1}{#2}{#3},
  "NET#1"+DR.{"NET#1-1"+0}!DR+L(.3)*+{#5}="NET#1-2"
  \restore\POS
  }

\newcommand{\lspine}[3]{%
  \save\POS
%  @(,
  @+, s0+<1em,1.5em>@+, s0+/u#3\vt/+/d1.5em/@+, s0+/l#2\hz/@+, 
  s0+/d#3\vt/@+, s0.{s0+/r#2\hz/}+R(.4)@+, s0+/u1.5em/@+,
  s6+<-1em,1.5em>@+,
  {s0 \ar@{-} 's1 's2 's3 's4 's5 's6 's7 s0},
  {s6.s4+C}.s1.s5="SPINE#1",
  s2.s3+C="SPINE#1-AUX",
  @-@-@-@-@-@-@-
%  @)
  \restore\POS
  }

\newcommand{\LSPINE}[5]{%
  \save\POS
  *+{#4}="SPINE#1-1",
  "SPINE#1-1"+U \lspine{#1}{#2}{#3},
  "SPINE#1-AUX".{"SPINE#1-1"+0}!DL*+{#5}="SPINE#1-2"
  \restore\POS
  }

\newcommand{\rspine}[3]{%
  \save\POS
%  @(,
  @+, s0+<-1em,1.5em>@+, s0+/u#3\vt/+/d1.5em/@+, s0+/r#2\hz/@+, 
  s0+/d#3\vt/@+, s0.{s0+/l#2\hz/}+L(.4)@+, s0+/u1.5em/@+,
  s6+<1em,1.5em>@+,
  {s0 \ar@{-} 's1 's2 's3 's4 's5 's6 's7 s0},
  {s6.s4+C}.s1.s5="SPINE#1",
  s2.s3+C="SPINE#1-AUX",
  @-@-@-@-@-@-@-
%  @)
  \restore\POS
  }

\newcommand{\RSPINE}[5]{%
  \save\POS
  *+{#4}="SPINE#1-1",
  "SPINE#1-1"+U \rspine{#1}{#2}{#3},
  "SPINE#1-AUX".{"SPINE#1-1"+0}!DR*+{#5}="SPINE#1-2"
  \restore\POS
  }


%\newcommand{\wtree}{%
%  \object\xybox{%
%    \newlength\un\un=1em
%    \POS 0*!C{\mathsf{w}},
%    <-1.25\un,.75\un>; <1.25\un,.75\un> **[thicker]\dir{-};
%    <0\un,-1.25\un> **[thicker]\dir{-};
%    <-1.25\un,.75\un> **[thicker]\dir{-}
%    }
%  }

\newcommand{\node}[1]{%
  \object[o]\xybox{*{#1},*[thicker]\cir<.7em>{}} %
}

\newcommand{\sfnode}[1]{%
  \object[o]\xybox{*{\mathsf{#1}},*[thicker]\cir<.7em>{}} %
}

%%% Tests
\newcommand{\testof}[1]{%
  #1 \ydash}
\newcommand{\proofof}[1]{%
  \testof{\pf{#1}}}
%\newcommand{\proofof}[1]{%
%  \ydash #1}
\newcommand{\ndderiv}[2]{%
  {#2} \ydash {#1}}

==> natdedsyst.tex <==
% !TEX root = ./main.tex
\section{Natural Deduction Systems}\label{sec:natdedsyst}
 In this section we define natural deduction systems for the class of logics we previously introduced. 
 
\rosso{Attenti: Nella definizione di formula (Sez \ref{sec:2seq}), non c'\`e $\bot$. Deve essere considerato un proposition symbol? (vedi restrizione su $\bot$-intro).
}
 
 \blue{
 Since, differently from the sequent calculus case, the natural deduction systems for \textbf{S4}, \textbf{T} and \textbf{D}, differ syntactically from the systems for \textbf{K} and \textbf{K4}, we separate the two classes of logics, calling \textbf{\textit{total}} the first one (\textbf{S4}, \textbf{T} and \textbf{D})  and \textbf{\textit{partial}} the second (\textbf{K} and \textbf{K4})
}
 
 \subsection{\blue{Total logics}}
 We start by defining the system $\mathbf{N_{S4}}$

\bigskip

The set of derivations from a set $\Gamma$ of assumptions is defined
as the least set that contains $\Gamma$ and is
closed under application of the following rules (where, as usual, a formula into square
brackets represents a discharged assumption):




\subsubsection*{Logical rules}
\begin{center}
   $\brule { \LT{\pf{A}{\alpha}}{  }} { \LT{\pf{B}{\alpha}}{ } } { \pf{A\land 
B}{\alpha} }
     {\ (\land I)} $
\qquad $\urule{\LT{\pf{A \land B}{\alpha}}{ }}{\pf{ A}{\alpha}}{\ (\land_1 E)}$ 
\qquad $\urule{\LT{\pf{A \land B}{\alpha}}{ }}{\pf{ B}{\alpha}}{\ (\land_2 E)}$
\end{center}

\bigskip

\begin{center}
   $\urule{\LT{\pf{A}{\alpha}}{ }}{\pf{A \lor B}{\alpha}}{\ (\lor_1 I)}$ \quad
   $\urule{\LT{\pf{B}{\alpha}}{ }}{\pf{A \lor B}{\alpha}}{\ (\lor_2 I)}$ \quad
   $\trule{\LT{\pf{A \lor B}{\alpha}}{ }} {\LT{\pf{C}{\beta}}{[\pf{A}{\alpha}]\  }}
   {\LT{\pf{C}{\beta}}{[\pf{B}{\alpha}]\ }} {\pf{C}{\beta}} {\ (\lor E)} $
\end{center}

\bigskip

\begin{center}
   $\urule { \LT{\pf{B}{\alpha}}{[\pf{A}{\alpha}]\  } } { \pf{A\to B}{\alpha} } {\ (\to 
I)} $ \qquad $
   \brule{\LT{\pf{A\to B}{\alpha}}{ }}{\LT{\pf{A}{\alpha}}{  }}{\pf{B}{\alpha}}{\ (\to 
E)} $
\end{center}

\bigskip


\begin{center}
   $\urule { \LT{\pf{\bot}{\beta}}{[\pf{\lnot A}{\alpha}]\  } } { \pf{A}{\alpha} } {\ 
(\bot_c)} $ \qquad $
   \urule { \LT{\pf{\bot}{\beta}  }{ } } { \pf{A}{\alpha} } {\ (\bot_i)}$
\end{center}

In rules $\bot_c$ and $\bot_i$ , the formula $A$ is a proposition symbol. In $\bot_i,$ when $A$
is $\bot$ we further require $\alpha\neq \beta.$

\bigskip

\begin{center}
   $ \urule { \LT{\pf{A}{\alpha\conc x}}{ } } { \pf{\Box A}{\alpha} } {\
     (\Box I) } $ \qquad $ %
   \urule { \LT{\pf{\Box A}{\alpha}}{ } } { \pf{A}{\alpha\conc \beta} } { (\Box E)
     } $
\end{center}

In the rule $\Box I$ $\alpha\conc x \not\in \iniz{\Gamma}$ where $\Gamma$ is the
set of assumptions on which $\pf{A}{\alpha\conc x}$ depends.

\bigskip

\begin{center}
   $ \urule { \LT{\pf{A}{\alpha\conc \beta}}{ } } { \pf{\Diamond A}{\alpha} } { \
     (\Diamond I) } $ \qquad $\brule{\LT{\pf{\Diamond A}{\alpha}}{ }}
   {\LT{\pf{C}{\beta}}{[\pf{A}{s\conc x}]\ }} {\pf{C}{\beta}} {\qquad (\Diamond 
E)} $
\end{center}

In the rule $\Diamond E$,  $\alpha\conc x \not\in \iniz{\Gamma}$ where $\Gamma$ is the
set of assumptions on which  $\pf{C}{\beta}$ depends, with the
exception of the discharged assumptions $\pf{A}{\alpha\conc x}$.

\bigskip

\begin{definition}[Proper Token]
We refer to the token $x$ that explicitly appears in any of the
rules $\Box I,\Diamond E$ as to the \textit{proper token} of the
corresponding rule. We say that a token \emph{is  proper  in a
derivation} if it is the proper token of some $\Box I,\Diamond E$
rule in the derivation.
\end{definition}

By token renaming we can we can prove the following (see~\cite[pag.
529]{tvdII} for a proof for variables):

\begin{proposition}\label{vc-cond}%
   Let $\Gamma\vdash_N \pf{A}{\alpha}$.  Then
   there exists a deduction of $\pf{A}{\alpha}$ from $\Gamma$ in the system
   $N$ such that
   \begin{enumerate}
   \item each proper token is the proper token of exactly one instance
     of $\Box I$ or $\Diamond E$ rule;
   \item the proper token of any instance of $\Box I$ rule occurs only
     in the sub-derivation above that instance of the rule;
   \item the proper token of any instance of $\Diamond E$
     rule occurs only in the sub-derivation above the minor premiss of
     that instance of the rule.
   \end{enumerate}
\end{proposition}


\begin{definition}[Token condition] A deduction satisfying conditions 1--3  of 
Proposition~\ref{vc-cond} is
said to satisfy  the \textit{token condition}.
\end{definition}

By  Proposition~\ref{vc-cond} we can always assume that all deductions
satisfy the token condition.




  We denote
by $\Pi\rep{\beta}{\gamma}$ the tree obtained by replacing each position $\alpha$ in
a deduction $\Pi$ with $\alpha\rep{\beta}{\gamma}$.


\begin{remark}\label{subst}   If the following hold
\begin{enumerate}
\item $\Pi$ is a deduction satisfying the token condition;
\item  $x$ is a token that is
not a  proper token of $\Pi;$
\item $\beta$ is a position not
containing any proper token of $\Pi;$
\end{enumerate}
then $\Pi\rep{\beta}{\gamma}$ is a deduction satisfying  the token condition.



Notice that if
$\Pi$ ends with $\bot_i$ and its  last formula is $\pf{\bot}{\alpha}$ for some 
$\alpha$
it might be that the corresponding  restriction in $\bot_i$ is
not satisfied after the substitution. In such a case by  $\Pi\rep{\beta}{\gamma}$ we 
mean the deduction obtained by
deleting,  after the substitution, the last -incorrect- application of 
$\bot_i.$
\end{remark}

We want to make sense of $\Pi\rep{\beta}{\gamma}$ even when the 
conditions of Remark~\ref{subst} are not satisfied. Notice that if $\Pi$ 
is a deduction satisfying the token condition, we can replace all proper tokens in $\Pi$ 
by new tokens so to obtain a deduction $\Pi'$ of the same formula 
from the same assumptions so that $t$ and $x$ satisfy all the 
conditions of Remark~\ref{subst}. Hence we define $\Pi\rep{\beta}{\gamma}$ as 
$\Pi'\rep{\beta}{\gamma}$ In the sequel we will implicitly assume that by $\Pi\rep{\beta}{\gamma}$ 
we actually mean $\Pi'\rep{\beta}{\gamma}$ for some $\Pi'$ as above.

{
\color{blue}
On the basis of $\mathbf{N_{S4}}$,  the natural deduction systems for the logics $T$, $D$,can be obtained 
by imposing suitable constraints on the application of   $\Box E$ and $\Diamond I$ rules, as shown in the following table.
\bigskip
\\
\begin{tabular}{|c|c|}
\hline 
\textbf{name of the calculus} & \textbf{constraints on  the rules $\Box E$ and $\Diamond I$}\\ 
\hline 
$\textbf{N}_{\textbf{S4}}$ & no constraints \\ 
\hline 
$\textbf{N}_{\textbf{T}}$  & $\beta=<\ >$ \\ 
\hline 
$\textbf{N}_{\textbf{D}}$  & $\beta$ is a singleton sequence $<z>$  \\ 
\hline 
\end{tabular} 

\fbox{relazione con i sequenti?}
\\
\fbox{occorre mostrare soundness e completezza, lo facciamo in relazione ai sequenti?}
\\
\fbox{...to be done...}
}



{ \color{blue}
\subsection{\blue{Partial logics}}

The main novelty with respect to the natural deduction system previously stated is in the use of a so called \textbf{existence} predicate for positions.

The \textbf{existence} predicate was introduced by D. Scott in the late seventieth \cite{} in order to deal with empty domains and consequently with partially defined terms.
Given a first order term $t$, $\ext{t}$ has the informal meaning \textit{$t$ is defined}.
An extensive treatment of \textbf{existence} predicate for natural deduction may be found in the two books of Troelstra and van Dalen "Constructivism in mathematics, vol. 1 and 2" (\cite{tavd}).

Since the logics \textbf{K} and \textbf{K4} could have partial accessibility relation (w.r.t. standard semantics) or equivalently partially defined positions (see the previously stated semantics~\ref{semantics-sequents}), it seems plausible to use the existence predicate for positions.

We augment the natural deduction system previously stated with the formulas $\ext{\alpha}$ which informal meaning is $\alpha$ denotes an existing object.

\textit{The formulas $\ext{\alpha}$ may be used only as premises in deductions.}


We  modify the rules for $\Box$ and $\Diamond$ in the following way:

\begin{center}
	$ \urule { \LT{\pf{A}{\alpha\conc x}}{[\ext{\alpha\conc x}] } } { \pf{\Box A}{\alpha} } {\
		(\Box I) } $ \qquad $ %
	\urule { \LT{\pf{\Box A}{\alpha}}{ }\ext{\alpha\conc \beta}} { \pf{A}{\alpha\conc \beta} } { (\Box E)
	} $
\end{center}

In the rule $\Box I$ $\alpha\conc x \not\in \iniz{\Gamma}$ where $\Gamma$ is the
set of assumptions on which $\pf{A}{\alpha\conc x}$ depends.

\bigskip

\begin{center}
	$ \urule { \LT{\pf{A}{\alpha\conc \beta}  }\qquad \ext{\alpha\conc \beta}{ } } { \pf{\Diamond A}{\alpha} } { \
		(\Diamond I) } $ \qquad $\brule{\LT{\pf{\Diamond A}{\alpha}}{ }}
	{\LT{\pf{C}{\beta}}{[\pf{A}{s\conc x}\quad \ext{\alpha\conc x}]\ }} {\pf{C}{\beta}} {\qquad (\Diamond 
		E)} $
\end{center}

In the rule $\Diamond E$,  $\alpha\conc x \not\in \iniz{\Gamma}$ where $\Gamma$ is the
set of assumptions on which  $\pf{C}{\beta}$ depends, with the
exception of the discharged assumptions $\pf{A}{\alpha\conc x}$.

The following table give the constraints for $\textbf{N}_{\textbf{K4}}$ and $\textbf{N}_{\textbf{K}}$.


\bigskip
\begin{tabular}{|c|c|}
	\hline 
	\textbf{name of the calculus} & \textbf{constraints on  the rules $\Box E$ and $\Diamond I$}\\ 
	\hline 
	$\textbf{N}_{\textbf{K4}}$ & $\beta$ is a non empty sequence \\ 
	\hline 
	$\textbf{N}_{\textbf{K}}$  & $\beta$ is a singleton sequence $<z>$  \\ 
	\hline 
\end{tabular} 

\fbox{relazione con i sequenti?}\\
\fbox{occorre mostrare soundness e completezza, lo facciamo in relazione ai sequenti?}\\
\fbox{occorre mostrare bene il ruolo del predicato di esisitenza}\\
\fbox{...to be done...}

}

==> normalization.tex <==
% !TEX root = ./main.tex
\section{Normalization}\label{sec:normalization}
\subsection{\blue{Total logics}}
We first introduce the following notation:

\begin{itemize}
\item[]$\vertil{
          \pf{B}{\beta} \\ \Pi \\ \pf{A}{\alpha}}$  to say that $\Pi$ is a 
deduction of formula
        $\pf{A}{\alpha}$ containing some occurrences of formula
        $\pf{B}{\beta}$ among its assumptions;


\item[]$\ded{\Pi}{R}{\pf{A}{\alpha}}$ to say that $\Pi$ is a deduction
   of formula $\pf{A}{\alpha}$ whose last rule is $R$.
\end{itemize}

In order to define the notion of \textit{normal form}  for a deduction, we must
explain what we mean by \textit{reduction sequence}. Therefore we first have to
introduce \textit{contractions}, that are crucial to the  definition of
\textit{reduction steps}. (See e.g~\cite{Girard:ptlc}.) 


\subsection*{Proper contractions}
The relation $\rhd$ of \textit{proper contractibility}  between 
deductions is defined as follows.

\rosso{Mancano le riduzioni di $\bot$ (non so se le considerate proprie o commutative).}

\def\uno{\DT{}{{\Pi}_1}{\pf{A}{\alpha}}}
\def\due{\DT{}{{\Pi}_2}{\pf{B}{\alpha}}}
\def\tre{\prova{\uno\quad\due \ }{\pf{A\land B}{\alpha}}{ }}
\def\quattro{\prova{\tre}{\pf{A}{\alpha}}{ }}

%$$\quattro\qquad \rhd \qquad \uno$$

\def\cinque{\prova{\tre}{\pf{B}{\alpha}}{ }}

%$$\cinque\qquad \rhd\qquad\due$$

\def\sei{\prova{\uno\ }{\pf{A\lor B}{\alpha}}{ }}
\def\sette{\DT{[\pf{A}{\alpha}]}{{\Pi}_2}{\pf{C}{\beta}}}
\def\otto{\DT{[\pf{B}{\alpha}]}{{\Pi}_3}{\pf{C}{\beta}}}
\def\nove{\prova{\sei\ \sette\ \otto\ }{\pf{C}{\beta}}{ }}
\def\dieci{\DT{\uno}{{\Pi}_2}{\pf{C}{\beta}}}


%$$\nove\qquad\rhd\qquad\dieci$$

\def\duebis{\DT{}{{\Pi}_1}{\pf{B}{\alpha}}}

\def\undici{\prova{\duebis}{\pf{A\lor B}{\alpha}}{ }}

\def\dodici{\prova{\undici\ \sette\ \otto\ }{\pf{C}{\beta}}{ }}
\def\tredici{\DT{\duebis}{{\Pi}_3}{\pf{C}{\beta}}}

%$$\dodici \qquad \rhd \qquad \tredici$$

\def\quattordici{\DT{[\pf{A}{\alpha}]}{{\Pi}_1}{\pf{B}{\alpha}}}
\def\quindici{\prova{\quattordici}{\pf{A\to B}{\alpha}}{ }}
\def\sedici{\DT{}{{\Pi}_2}{\pf{A}{\alpha}}}
\def\diciassette{\prova{\quindici\ \sedici}{\pf{B}{\alpha}}{ }}
\def\diciotto{\DT{\sedici}{{\Pi}_1}{\pf{B}{\alpha}}}

\bigskip

%$$\diciassette \qquad\rhd\qquad \diciotto$$

\def\venti{\DT{}{\Pi}{\pf{A}{s\oplus 1}}}
\def\ventuno{\prova{\venti}{\pf{ A}{\alpha}}{}}
\def\ventidue{\prova{\ventuno}{\pf{A}{s\oplus 1}}{}}

\bigskip

%$$\ventidue \qquad\rhd\qquad \venti$$

\bigskip

\def\ventitre{\DT{}{\Pi}{\pf{A}{\alpha \conc x}}}
\def\ventiquattro{\prova{\ventitre}{\pf{\Box A}{\alpha}}{ }}
\def\venticinque{\prova{\ventiquattro}{\pf{A}{\alpha \conc \beta}}{ }}
\def\ventisei{\DT{}{{\Pi}\rep{\alpha\conc x}{\alpha\conc \beta}}{\pf{A}{\alpha \conc \beta}}}

%$$\venticinque\qquad\rhd\qquad\ventisei$$

\def\ventisette{\DT{}{{\Pi}_1}{\pf{A}{\alpha \conc \beta}}}
\def\ventotto{\prova{\ventisette}{\pf{\Diamond A}{\alpha}}{ }}
\def\ventinove{\DT{[\pf{A}{\alpha \conc x}]}{{\Pi}_2}{\pf{C}{\gamma}}}
\def\trenta{\prova{\ventotto\ \ventinove}{\pf{C}{\gamma}}{ }}

\def\trentuno{\DT{}{{\Pi}_1}{\pf{A}{\alpha \conc \beta}}}
\def\trentadue{\DT{\trentuno}{{\Pi}_2\rep{\alpha\conc x}{\alpha\conc\beta}}{\pf{C}{\gamma}}}

%$$\trenta \qquad\rhd\qquad \trentadue$$

\def\trentatre{\DT{}{{\Pi}_1}{\pf{A}{\alpha}}}
\def\trentaquattro{\DT{[\pf{A}{\alpha \conc x}]}{{\Pi}_2}{\pf{A}{s\oplus 
<1,x>}}}
\def\trentacinque{\prova{\trentatre\ \trentaquattro}{\pf{A}{\alpha}}{}}

\def\trentacinquebis{\prova{\trentatre\
     \trentaquattro}{\pf{A}{s\oplus(t\oplus 1)}}{}}

\def\trentasei{\prova{\trentatre\
     \trentaquattro}{\pf{A}{\alpha \conc \beta}}{}}


\def\trentasette{\DT{\trentasei}{\Pi_2\rep{\beta}{\gamma}}{\pf{A}{s\oplus(t\oplus 1)}}}
%\def\trentotto{\DT{\trentasette}{{\Pi}_2[<<k-1;\emptyset>/x]}{<n+k;S>:A}}

%$$\trentacinque  \qquad\rhd\qquad \trentatre$$
%$$\trentacinquebis  \qquad\rhd\qquad \trentasette$$


\begin{tabular}{ll}
$ \quattro \quad \rhd\quad  \uno $
&\hspace{2ex}
$ \cinque  \quad\rhd \quad \due  $
\\ & \\
$\nove  \quad\rhd \quad \dieci$
&\hspace{2ex}
$\dodici \quad\rhd \quad \tredici $
\\ & \\
$\diciassette  \quad\rhd \quad\diciotto $
&\hspace{2ex}

%$ \ventidue  \quad\rhd \quad \venti $
\\ & \\
$\venticinque \quad\rhd \quad\ventisei$
&\hspace{2ex}
$\trenta  \quad\rhd \quad\trentadue $
%\\ & \\
%$\trentacinque \quad\rhd \quad\trentatre$%
%&\hspace{2ex}
%$\trentacinquebis \quad\rhd \quad\trentasette$
\end{tabular}


\subsection*{Commutative contractions}

In this subsection, by 

\centerline{\raisebox{4ex}{$\prova{\DT{}{\Pi_1}{\pf{C}{\beta}}\quad
       \Pi_2}{\pf{D}{\gamma}}{\ R}$}}
\noindent we denote  a deduction ending with an  elimination 
rule $R$ whose major premiss  is formula
$\pf{C}{\beta}$.

\bigskip

We further extend the relation $\rhd$ by adding the
following \textit{commutative contractions}:

\newcommand{\sureg}[2]{\prova{ #1\quad {{\Pi}_{#2}}}{\pf{D}{\gamma}}{\ R}}
\newcommand{\surego}[2]{\prova{ #1\quad {{\Pi}_{#2}}}{\pf{A}{\alpha}}{\ R}}

\def\quaranta{\DT{}{{\Pi}_1}{\pf{A\lor B}{\alpha}}}
\def\quarantuno{\DT{[\pf{A}{\alpha}]}{{\Pi}_2}{\pf{C}{\beta}}}
\def\quarantadue{\DT{[\pf{B}{\alpha}]}{{\Pi}_3}{\pf{C}{\beta}}}
\def\quarantatre{\prova{\quaranta\ \quarantuno\ 
\quarantadue}{\pf{C}{\beta}}{}}
\def\quarantaquattro{\sureg{\quarantatre}{4}}

\def\quarantacinque{\sureg{\quarantuno}{4}}
\def\quarantasei{\sureg{\quarantadue}{4}}
\def\quarantasette{\prova{\quaranta\ \quarantacinque\
     \quarantasei}{\pf{D}{\gamma}}{ }}



$$\quarantaquattro  \quad\rhd\quad \quarantasette$$

\bigskip

\def\cinquanta{\DT{}{{\Pi}_1}{\pf{\Diamond A}{\alpha}}}
\def\cinquantuno{\DT{[\pf{A}{\alpha \conc x}]}{{\Pi}_2}{\pf{C}{\beta}}}
\def\cinquantadue{\prova{\cinquanta\ \cinquantuno}{\pf{C}{\beta}}{}}
\def\cinquantatre{\sureg{\cinquantadue}{3}}
\def\cinquantaquattro{\sureg{\cinquantuno}{3}}
\def\cinquantacinque{\prova{\cinquanta\ \cinquantaquattro}{\pf{D}{\gamma}}{}}

\def\cento{\DT{}{{\Pi}_1}{\pf{\Diamond B}{t}}}
\def\centouno{\DT{[\pf{B}{t\oplus x}]}{{\Pi}_2}{\pf{C}{u}}}
\def\centodue{\prova{\cento\ \centouno}{\pf{C}{u}}{}}
\def\centotre{\surego{\centodue}{3}}
\def\centoquattro{\surego{\centouno}{3}}
\def\centocinque{\prova{\cento\ \centoquattro}{\pf{A}{\alpha}}{}}

\def\duecento{\DT{}{{\Pi'}_1}{\pf{\Diamond B}{t}}}
\def\duecentodue{\prova{\duecento\ \centouno}{\pf{C}{u}}{}}


$$\cinquantatre \quad\rhd\quad \cinquantacinque$$

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\vspace{0.5cm}

\begin{remark} It is easy to verify that  contractions transform 
deductions into deductions.  Furthermore they all preserve the token 
condition.
\end{remark}

\begin{definition}\label{def:red}
  \begin{enumerate}
\item  The relation $\red$ of \textit{immediate reducibility}  between 
deductions is defined
   as follows: $\Pi_1\red \Pi_2$ if and only if there exist deductions  
$\Pi_3$ and
   $\Pi_4$ such that $\Pi_3\rhd\Pi_4$ and $\Pi_2$ is obtained by
   replacing $\Pi_3$ with $\Pi_4$ in $\Pi_1$.
  \item The relation  $\rred$ of \textit{reducibility} is the transitive 
and reflexive closure of $\red$.
\end{enumerate}
\end{definition}




\begin{definition} Let $\Pi$ be a deduction. 
   A \textit{reduction sequence of $\Pi$ of length $I\leq\omega$} is a 
sequence
   of deductions $(\Pi_i)_{i \lt I}$ such 
   that $\Pi_0=\Pi$ and $\Pi_{i-1}\red \Pi_i$ for all $0 \lt i \lt I$.
\end{definition}



\begin{definition} A deduction $\Pi$ is
\begin{enumerate}
   \item  \textit{strongly  normalizing}
%(and we   will write $SN[\Pi]$),
   if all  reduction sequences of $\Pi$ are  finite;
\item in \textit{normal form}
%(and we will   write $NF[\Pi]$)
   if there is no deduction $\Pi'$ such that $\Pi\red\Pi'$.
\end{enumerate}
\end{definition}

\begin{definition}
\begin{enumerate}
\item A finite sequence $(\pf{A_i}{\alpha})_{i\leq m} $ of formulas in a
   deduction is a \textit{segment} if:
   \begin{enumerate}
   \item for all $i\lt m$, $\pf{A_i}{\alpha}$ is immediately above $\pf{A_{i+1}}{\alpha}$;
   \item $\pf{A_0}{\alpha}$ is  not a conclusion of $\lor E$ or $\Diamond E$;
   \item  $\pf{A_m}{\alpha}$ is not a minor premiss of $\lor E$ or $ \Diamond 
E$;
   \item for all $i \lt m$, $\pf{A_i}{\alpha}$ is a minor premiss of $\lor E$
     or $ \Diamond E$.
   \end{enumerate}

  % (as a trivial consequence all the $A_i$ are instances of the same 
%formula.)

\item A segment in a deduction is an \textit{endsegment} if its last 
formula is the last formula of  the deduction.
\end{enumerate}

\end{definition}

Given a deduction $\ded{\Pi}{R}{\pf{A}{\alpha}},$ with little abuse of 
language  we will say that a deduction $\Pi'$
   is a  \textit{(main) premiss of rule} $R$ to mean that
$\Pi'$ is a sub-deduction of $\Pi$ whose end-formula is a (main)  premiss 
of the displayed application of $R.$

We will use the notation


\begin{itemize}
\item[]$mp_{\Pi}[R]$ for the deduction that is the main premiss of rule 
$R$ in $\Pi;$
\item[]$pr_{\Pi}[R]$ for the set of deductions that are premisses of 
rule $R$ in
   $\Pi;$

(When there is no ambiguity  we will omit the subscripts.)

\item[]$h[\Pi]$ for  the \textit{height} (standardly defined) of the
   deduction $\Pi;$
\item[]$rd[\Pi]$ for the maximum length  of reduction sequences
   of $\Pi.$
\end{itemize}

We can prove SN by reducing the problem  to normalization of full propositional intuitionistic logic.

\subsection{A forgetful embedding}

\rosso{anche qui manca $\bot$.}

Let us consider the following function $(\ )^*: \pwff \to \wff$ so defined:

\[
\begin{array}{rcl}
(\pf{p}{})^*  &  =  &  p\\
(\pf{\bot}{})^*  &  =  &  \bot\\
(\pf{\neg A}{})^*  &  =  &  \neg (\pf{A}{})^* \\
(\pf{A\wedge B}{})^*  &  =  &  (\pf{A}{})^* \wedge (\pf{B}{})^* \\
(\pf{A\vee B}{})^*  &  =  &  (\pf{A}{})^* \vee (\pf{B}{})^* \\
(\pf{A\to B}{})^*  &  =  &  (\pf{A}{})^* \to (\pf{B}{})^* \\
(\pf{\Box A}{})^*  &  =  &  (\pf{A}{})^* \\
(\pf{\Diamond A}{})  &  =  &  (\pf{A}{})^* \\
\end{array}
\]

Now let us consider the following forgetful transformation $(\ )^*$ for deductions (we give only some case)

$$
\left(
\prova{ % premessa
  \DT{ 
  [\pf{A}{\alpha}] 
  }
  {\Pi_1}
  {\pf{B}{\alpha}}
  }
  { % conclusione
  \pf{A\to B}{\alpha}
  }
  { • } %nome 
  \right)^*
  =
  \prova{ % premessa
  \DT{ 
 [ \pf{(A)^*}{}] 
  }
  {\!\! (\Pi_1)^*}
  {\pf{(B)^*}{}}
  }
  { % conclusione
  \pf{(A\to B)^*}{}
  }
  { • } %nome 
\qquad
\left(
\prova{ % premessa
  \DT{}
  {\Pi_1}
  {\pf{A\to B}{\alpha}}
\quad
\DT{}
  {\Pi_2}
  {\pf{A}{\alpha}}
  }
  { % conclusione
  \pf{B}{\alpha}
  }
  { • } %nome 
  \right)^*
  =
  \prova{ % premessa
  \DT{}
  {\!\!\!(\Pi_1)^*}
  {\pf{(A\to B)^*}{}}
\quad
\DT{}
  {\!\!\!(\Pi_2)^*}
  {\pf{(A)^*}{}}
  }
  { % conclusione
  \pf{(B)^*}{}
  }
  { • } %nome 
$$

$$
\left(
\prova{ % premessa
  \DT{}{\Pi}{\pf{A}{\alpha\conc x}}
  }
  { % conclusione
  \pf{\Box A}{\alpha}
  }
  { • } %nome 
  \right)^*
  =
  \DT{}{\!\!\!(\Pi)^*}{(A)^*}
  \quad
  \left(
\prova{ % premessa
  \DT{}{\Pi}{\pf{\Box A}{\alpha}}
  }
  { % conclusione
  \pf{\Box A}{\alpha\conc \beta}
  }
  { • } %nome 
  \right)^*
  =
  \DT{}{\!\!\!(\Pi)^*}{(A)^*}
$$

$$
\left(
\prova{ % premessa
  \DT{}{\Pi}{\pf{A}{\alpha\conc \beta}}
  }
  { % conclusione
  \pf{\Diamond A}{\alpha}
  }
  { • } %nome 
  \right)^*
  =
  \DT{}{\!\!\!(\Pi)^*}{(A)^*}
  \quad
  \left(
\prova{ % premessa
  \DT{}{\Pi_1}{\pf{\Diamond A}{\alpha}}
  \DT{[ \pf{A}{\alpha\conc x}] }{ \Pi_2}{ \pf{C}{\beta}}
  }
  { % conclusione
  \pf{C}{\beta}
  }
  { • } %nome 
  \right)^*
  =
  \DT{
  \DT{}{\!\!\!(\Pi_1)^*}{(A)^*}
  }
  {(\Pi_2)^*}
  {(C)^*}
$$

Let $\rhd_p$ and $\red_p$ the standard contractibility and reducibility reduction for $NJ$

\begin{proposition}\label{prop:emb}
\begin{enumerate}
\item If $\Pi_1\rhd \Pi_2$ by means of a modal contraction then $(\Pi_1)^*= (\Pi_1)^*$;
\item If $\Pi_1\rhd \Pi_2$ by means of a non modal contraction then $(\Pi_1)^*\rhd_p (\Pi_1)^*$; by using the same kind of contraction
\end{enumerate}
\end{proposition}

\blu{
\begin{theorem}[strong normalization]\label{theor:SN}
Let $\sys\in\mathbf{\{{KD}, {KT},{S4}\}}$. Each proof  $\Pi$ in $\textbf{N}_{\sys}$ is strongly normalizing.
\end{theorem}	
\begin{proof}
Let us suppose that $\Pi$ has an infinite reduction sequences. It is immediate to observe that such a reduction cannot be  definitively composed by modal reduction, since such a reduction reduce the size of the proof.
This means that such a reduction must contains a subsequence of non modal reductions. But this means that (corollary of proposition~\ref{prop:emb}) $(\Pi)^*$ is not SN, absurd.
\end{proof}
}

{\color{blue}
\subsection{\blue{Partial logics}}

The reduction involving modal rules must be trivially adapted to deal  with existence predicate.

%%%%%%%%%%%%%%
%%%%%%%%%%%%%%

\def\uno{\DT{}{{\Pi}_1}{\pf{A}{\alpha}}}
\def\due{\DT{}{{\Pi}_2}{\pf{B}{\alpha}}}
\def\tre{\prova{\uno\quad\due \ }{\pf{A\land B}{\alpha}}{ }}
\def\quattro{\prova{\tre}{\pf{A}{\alpha}}{ }}

%$$\quattro\qquad \rhd \qquad \uno$$

\def\cinque{\prova{\tre}{\pf{B}{\alpha}}{ }}

%$$\cinque\qquad \rhd\qquad\due$$

\def\sei{\prova{\uno\ }{\pf{A\lor B}{\alpha}}{ }}
\def\sette{\DT{[\pf{A}{\alpha}]}{{\Pi}_2}{\pf{C}{\beta}}}
\def\otto{\DT{[\pf{B}{\alpha}]}{{\Pi}_3}{\pf{C}{\beta}}}
\def\nove{\prova{\sei\ \sette\ \otto\ }{\pf{C}{\beta}}{ }}
\def\dieci{\DT{\uno}{{\Pi}_2}{\pf{C}{\beta}}}


%$$\nove\qquad\rhd\qquad\dieci$$

\def\duebis{\DT{}{{\Pi}_1}{\pf{B}{\alpha}}}

\def\undici{\prova{\duebis}{\pf{A\lor B}{\alpha}}{ }}

\def\dodici{\prova{\undici\ \sette\ \otto\ }{\pf{C}{\beta}}{ }}
\def\tredici{\DT{\duebis}{{\Pi}_3}{\pf{C}{\beta}}}

%$$\dodici \qquad \rhd \qquad \tredici$$

\def\quattordici{\DT{[\pf{A}{\alpha}]}{{\Pi}_1}{\pf{B}{\alpha}}}
\def\quindici{\prova{\quattordici}{\pf{A\to B}{\alpha}}{ }}
\def\sedici{\DT{}{{\Pi}_2}{\pf{A}{\alpha}}}
\def\diciassette{\prova{\quindici\ \sedici}{\pf{B}{\alpha}}{ }}
\def\diciotto{\DT{\sedici}{{\Pi}_1}{\pf{B}{\alpha}}}

\bigskip

%$$\diciassette \qquad\rhd\qquad \diciotto$$

\def\venti{\DT{}{\Pi}{\pf{A}{s\oplus 1}}}
\def\ventuno{\prova{\venti}{\pf{ A}{\alpha}}{}}
\def\ventidue{\prova{\ventuno}{\pf{A}{s\oplus 1}}{}}

\bigskip

%$$\ventidue \qquad\rhd\qquad \venti$$

\bigskip

%\def\PiA{
%	 \DT{\ext{\alpha\conc x} }{\Pi}{}
%}

\def\ventitre{\DT{[\ext{\alpha\conc x}]}{\Pi}{\pf{A}{\alpha \conc x}  }}

\def\ventiquattro{\prova{\ventitre}{\pf{\Box A}{\alpha}}{ } \ext{\alpha\conc\beta}  }

\def\venticinque{\prova{\ventiquattro}{\pf{A}{\alpha \conc \beta}  }{ }}

\def\ventisei{\DT{\ext{\alpha\conc\beta}}{{\Pi}\rep{\alpha\conc x}{\alpha\conc \beta}}{\pf{A}{\alpha \conc \beta}}}

%$$\venticinque\qquad\rhd\qquad\ventisei$$

\def\ventisette{\DT{}{{\Pi}_1}{
		\pf{A}{\alpha \conc \beta}   
}}

\def\ventotto{\prova{\ventisette \ext{\alpha\conc \beta}}{\pf{\Diamond A}{\alpha}}{ }}

\def\ventinove{\DT{[\pf{A}{\alpha \conc x} \quad \ext{\alpha\conc x}]}{{\Pi}_2}{\pf{C}{\gamma}}}


\def\trenta{\prova{\ventotto\ \ventinove}{\pf{C}{\gamma}}{ }}

\def\trentuno{\DT{}{{\Pi}_1}{
		\pf{A}{\alpha \conc \beta}
	}
}
\def\trentadue{\DT{\trentuno  
	\ext{\alpha\conc\beta}
}{{\Pi}_2\rep{\alpha\conc x}{\alpha\conc\beta}}{\pf{C}{\gamma}}}

%$$\trenta \qquad\rhd\qquad \trentadue$$

\def\trentatre{\DT{}{{\Pi}_1}{\pf{A}{\alpha}}}
\def\trentaquattro{\DT{[\pf{A}{\alpha \conc x}]}{{\Pi}_2}{\pf{A}{s\oplus 
			<1,x>}}}
\def\trentacinque{\prova{\trentatre\ \trentaquattro}{\pf{A}{\alpha}}{}}

\def\trentacinquebis{\prova{\trentatre\
		\trentaquattro}{\pf{A}{s\oplus(t\oplus 1)}}{}}

\def\trentasei{\prova{\trentatre\
		\trentaquattro}{\pf{A}{\alpha \conc \beta}}{}}


\def\trentasette{\DT{\trentasei}{\Pi_2\rep{\beta}{\gamma}}{\pf{A}{s\oplus(t\oplus 1)}}}
%\def\trentotto{\DT{\trentasette}{{\Pi}_2[<<k-1;\emptyset>/x]}{<n+k;S>:A}}




\def\cinquanta{\DT{}{{\Pi}_1}{\pf{\Diamond A}{\alpha}}}
\def\cinquantuno{\DT{[\pf{A}{\alpha \conc x}\quad 
		\ext{\alpha\conc x}]}{{\Pi}_2}{\pf{C}{\beta}}}
\def\cinquantadue{\prova{\cinquanta\ \cinquantuno}{\pf{C}{\beta}}{}}
\def\cinquantatre{\sureg{\cinquantadue}{3}}

\def\cinquantaquattro{\sureg{\cinquantuno}{3}}
\def\cinquantacinque{\prova{\cinquanta\ \cinquantaquattro}{\pf{D}{\gamma}}{}}


%%%%%%%%%%%%%
%%%%%%%%%%%%%


$$\venticinque \quad\rhd \quad\ventisei$$

$$\trenta  \quad\rhd \quad\trentadue $$

$$\cinquantatre \quad\rhd\quad \cinquantacinque$$

Let us \textit{extend} the forgetful transormation above stated, by simply erasing each occurrence of the existence predicate. By means of the same argument used for proof of theorem~\ref{theor:SN}
we obtain  the following strong normalization theorem.

\blu{
	\begin{theorem}[strong normalization]
		Let $\sys\in\mathbf{\{{K},{K4}\}}$. Each proof  $\Pi$ in $\textbf{N}_{\sys}$ is strongly normalizing.
	\end{theorem}
}

}
